Divergence Free Polar Wavelets for the Analysis and Representation of Fluid Flows

We present a Parseval tight wavelet frame for the representation and analysis of velocity vector fields of incompressible fluids. Our wavelets have closed form expressions in the frequency and spatial domains, are divergence free in the ideal, analytic sense, have a multi-resolution structure and fast transforms, and an intuitive correspondence to common flow phenomena. Our construction also allows for well defined directional selectivity, e.g. to model the behavior of divergence free vector fields in the vicinity of boundaries or to represent highly directional features like in a von K\'arm\'an vortex street. We demonstrate the practicality and efficiency of our construction by analyzing the representation of different divergence free vector fields in our wavelets.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

\begin{figure}
  \includegraphics[trim={1740pt 280pt 0pt 410pt},clip,width=\columnwidth]{ball.pdf}
  \caption{The classical fluid flow around a ball with a von K{\'a}rm{\'a}n vortex street. Data set from an FEM simulation (top) and wavelet reconstruction with three levels (bottom). Slight differences, e.g. on the left, are a consequence of the input data only being approximately divergence free. The right column depicts basis function coefficients on the finest level for the orientations in the inset in the vicinity of the ball. The plots validate that our directional wavelets indeed provide good angular selectivity and yield sparse representations.}
  \label{fig:ball}
\end{figure}

We introduced a Parseval tight frame of divergence free wavelets that, next to other desirable properties, provides well defined angular localization.
We also showed that the wavelets have analytic expressions in frequency and space and that the filter taps for the fast transform can be computed in closed form and to arbitrary precision.
The beneficial properties of the wavelets result from a construction that intrinsically ensures that they are tangential to the frequency sphere, and hence divergence free in space, and from using windows functions defined in spherical coordinates.
Our windows are bandlimited in the frequency domain, so that the wavelets do not have compact support in space.
This complicates working with the wavelets in the spatial domain and, for example, the filter taps for the fast transform are typically truncated.
Nonetheless, our construction yields a practical implementation of divergence-free, directional wavelets and we validated this with numerical experiments.

In future work, we would like to perform more extensive numerical experiments and investigate more applications of our construction.
We are currently working on a local spectral fluid simulator that retains the advantages of spectral methods but allows for spatial adaptivity.
In this work we also exploit the closed form expression for $\nabla \times \vec{\psi}_s$, i.e. that vorticity can be computed analytically.
We would also like to investigate in more detail the two different types of boundary functions that we constructed in two dimensions and to better understand to which flow feature these correspond.
In three dimensions, the boundary functions also need to be investigated in more detail.


==> construction.tex <==
\section{Divergence Free Polar Wavelets}
\label{sec:construction}

We begin the section by recalling the scalar polar wavelets recently introduced by Unser and co-workers~\cite{Chenouard2012,Unser2013,Ward2014}.
We then detail the construction of our divergence free wavelets in two dimensions before turning to the $3$-dimensional setting.
In Sec.~\ref{sec:div_free:fast_transform} we detail the computation of the filter taps required for the fast transform.
Our conventions have been relegated to Appendix~\ref{sec:conventions}.
%%Our construction builds on the unified framework for steerable and directional wavelets that was recently introduced by Unser and co-workers~\cite{Chenouard2012,Unser2013,Ward2014}  and which we will refer to as polar wavelets~\cite{Lessig2018a}.
%%Hence, we briefly discuss these in Sec.~\ref{sec:construction:scalar}
%%In Sec.~\ref{sec:construction:2d}
%We will then introduce our frame of divergence free wavelets in two dimensions and study its properties.
%Sec.~\ref{sec:construction:3d} is devoted to the $3$-dimensional setting.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Scalar Polar Wavelet}
\label{sec:construction:scalar}

Polar wavelets~\cite{Chenouard2012,Unser2013,Ward2014,Lessig2018a} are separable in spherical coordinates in the Fourier domain $\mathbb{R}_{\xi}^d$.
They are hence given by $\hat{\psi}_s(\xi) = \hat{\gamma}_s(\bar{\xi}) \, \hat{h}_s(\vert \xi \vert)$ where $\hat{\gamma}_s(\bar{\xi})$ is an angular window over directions and $\smash{\hat{h}_s(\vert \xi \vert)}$ a radial one.
The multi-index $s = (j_s,k_s,t_s)$ describes the scale, position and orientation of the wavelets and, without loss of generality, we assume there are $M_j$ different orientations generated as rotations of one angular mother window $\hat{\gamma}(\bar{\xi})$.


%\begin{figure*}
%  \begin{center}
%  \includegraphics[width=0.1375\textwidth]{psihat_ns_j0_ko0}
%  \hspace{5pt}
%  \includegraphics[width=0.1375\textwidth]{psihat_ns_j1_ko0}
%  \hspace{5pt}
%  \includegraphics[width=0.1375\textwidth]{psihat_ns_j2_ko0}
%  \hspace{5pt}
%  \includegraphics[width=0.1375\textwidth]{psihat_ns_j3_ko0}
%  \hspace{5pt}
%  \includegraphics[width=0.1375\textwidth]{psihat_ns_j4_ko0}
%  \hspace{5pt}
%  \includegraphics[width=0.1375\textwidth]{psihat_fs_j4_ko0}
%  \\
%  \includegraphics[width=0.1375\textwidth]{psi_ns_j0_ko0}
%  \hspace{5pt}
%  \includegraphics[width=0.1375\textwidth]{psi_ns_j1_ko0}
%  \hspace{5pt}
%  \includegraphics[width=0.1375\textwidth]{psi_ns_j2_ko0}
%  \hspace{5pt}
%  \includegraphics[width=0.1375\textwidth]{psi_ns_j3_ko0}
%  \hspace{5pt}
%  \includegraphics[width=0.1375\textwidth]{psi_ns_j4_ko0}
%  \hspace{5pt}
%  \includegraphics[width=0.1375\textwidth]{psi_fs_j4_ko0}
%  \end{center}
%  \caption{Wavelets in the Fourier (top) and spatial domains (bottom) with a curvelet-like coupling between the radial and angular scaling. The second to fourth column show no-slip boundary functions and the last one a free slip one. Note the differences in the orientations of the vector fields in frequency and space.}
%  \label{fig:psis:2d}
%\end{figure*}

\begin{figure}
  \begin{center}
  \includegraphics[width=0.24\columnwidth]{psihat_ns_j0_ko0}
  \includegraphics[width=0.24\columnwidth]{psihat_ns_j1_ko0}
  \includegraphics[width=0.24\columnwidth]{psihat_ns_j3_ko0}
  \includegraphics[width=0.24\columnwidth]{psihat_fs_j3_ko0}
  \\
  \includegraphics[width=0.24\columnwidth]{psi_ns_j0_ko0}
  \includegraphics[width=0.24\columnwidth]{psi_ns_j1_ko0}
  \includegraphics[width=0.24\columnwidth]{psi_ns_j3_ko0}
  \includegraphics[width=0.24\columnwidth]{psi_fs_j3_ko0}
  \end{center}
  \caption{Divergence free wavelets in the Fourier (top) and spatial domains (bottom). The left columns shows an isotropic function that can be interpreted as an isolated vortex. The remaining ones provide examples of directional wavelets for the horizontal orientation with different angular localizations and for shearing- (middle two columns) and streaming-like flows (right column).}
  \label{fig:psis:2d}
\end{figure}

In two dimensions, the angular window is naturally written as a Fourier series.
Polar wavelets are there hence given by
\begin{align}
  \label{eq:polarlets:2d}
  \hat{\psi}_{s}(\xi)
  = \! \Bigg( \sum_m \beta_{m}^{j_s,t_s} \, e^{i m \theta_{\xi}} \Bigg) \hat{h}\big(2^{-j_s} \vert \xi \vert \big) \, e^{-i \langle \xi , 2^{-j_s} k_s \rangle}
\end{align}
with $\beta_{n}^{j_s,t_s} = \beta_{n}^{j_s} \, e^{-i n t_s (2\pi / M_{j_s})}$, i.e. the different orientations are obtained by rotating a fixed, possibly level-dependent window function.
% and $\theta_{\xi}$ being the angular variable in polar coordinates.
In the simplest case $\beta_n = \delta_{n 0}$ and one obtains isotropic functions.
The polar wavelets defined by Eq.~\ref{eq:polarlets:2d} also have a closed form expression in the spatial domain~\cite{Unser2013,Lessig2018a}.
% given by
%\begin{align}
%  \label{eq:polarlets:2d:space}
%  \psi_{s}(x)
%  = \frac{2^j}{2\pi} \Bigg( \sum_{m} i^m \, \beta_{m}^{j_s,t_s} \, e^{i m \theta_{x}} \Bigg)  h_m( 2^{j} \vert \xi - k \vert )
%\end{align}
%\end{subequations}
%with $h_n(r)$ being the $n^{\textrm{th}}$-order Hankel transform of $\hat{h}(\vert \xi \vert)$ which has an analytic solution for the Portilla-Simoncelli~\cite{Portilla2000}  window.
% Eq.~\ref{eq:polarlets:2d} shows that the angular window $\hat{\gamma}(\theta_{\xi})$ is in fact invariant under the inverse Fourier transform, up to the factor if $i^n = e^{i n \pi / 2}$ which implements a rotation by $\pi / 2$.

The construction in two dimensions carries over to the $3$-dimensional setting when the Fourier series is replaced by a spherical harmonics expansion.
In $\mathbb{R}^3$, polar wavelets are hence defined by
\begin{align}
  \label{eq:polarlets:3d}
  \hat{\psi}_{s}(\xi)
  = \Bigg( \sum_{l,m} \kappa_{lm}^{j_s,t_s} \, y_{lm}(\bar{\xi}) \Bigg) \hat{h}(2^{-j_s} \vert \xi \vert) \, e^{-i \langle \xi , 2^{-j_s} k_s \rangle}
\end{align}
and one can again derive a closed form expression in the spatial domain~\cite{Lessig2018a}.
%and their closed form expression in the spatial domain is
%\begin{align}
%	\psi_s(x) = \frac{2^{3j/2}}{(2\pi)^{3/2}} \Bigg( \!	\sum_{l,m} i^l \, \kappa_{lm}^{j_s,t_s} \, y_{lm}(\bar{x}) \! \Bigg) h_l(\vert 2^{j_s} x \! - \! k_s \vert) .
%\end{align}
%\end{subequations}
%The radial window functions $h_l(r)$ are generalized Hankel transforms of $\hat{h}(\vert \xi \vert)$ for the spherical Bessel function $j_l(r)$. These have again closed form expressions for the Portilla-Simoncelli window.

Under suitable admissibility conditions for $\hat{h}(\vert \xi \vert)$ and the coefficients $\beta_{j,n}^t$ and $\kappa_{lm}^{jt}$ defining the angular window functions $\hat{\gamma}(\bar{\xi})$, the wavelets in Eq.~\ref{eq:polarlets:2d} and Eq.~\ref{eq:polarlets:3d} form tight frames for $L_2(\mathbb{R}^2)$~\cite{Unser2013} and $L_2(\mathbb{R}^3)$~\cite{Ward2014}, respectively.
As usual, in practice on typically uses scaling functions, denoted as $\phi(x)$, on a coarsest level to represent the low frequency part of a signal.
We refer to the original works for more details.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Divergence free polar wavelets in 2D}
\label{sec:construction:2d}

For a $2$-dimensional vector field to be divergence free it has to be tangential to the circle $S_{\vert \xi \vert}^1$ in frequency space for every radius $\vert \xi \vert$ for which it is defined.
%The canonical basis for such vector fields is the angular coordinate vector $\vec{e}_{\theta_{\xi}}$, see again the inset figure.
These vector fields are hence naturally described in polar coordinates since then the radial vector component with respect to $\vec{e}_r$ has to vanish and only the angular one with respect to $\vec{e}_{\theta}$ can be nonzero.
A divergence free polar mother wavelet thus has to have the form
\label{eq:psi:divfree:2d}
\begin{align}
  \label{eq:psi:divfree:2d:frequency}
	\hat{\vec{\psi}}(\xi)
	= - i \, \hat{\gamma}(\theta_{\xi}) \, \hat{h}(\vert \xi \vert) \, \vec{e}_{\theta}
	= - i \Bigg( \! \sum_{n = -N}^N \beta_n \, e^{i n \theta_{\xi}} \Bigg) \, \hat{h}(\vert \xi \vert) \, \vec{e}_{\theta}
\end{align}
where the factor of $-i$ ensures that $\hat{\vec{\psi}}(\xi)$ is real-valued in space.
% Since the window functions are defined in polar coordinates, the inverse Fourier transform of Eq.~\ref{eq:psi:divfree:2d:frequency} can be computed in closed form.
To obtain the spatial representation, we write $\vec{e}_{\theta_{\xi}}$ as $\vec{e}_{\theta_{\xi}} = (\sin{\theta_{\xi}}, -\cos{\theta_{\xi}})$ with respect to canonical Cartesian coordinates so that we can compute the inverse transform independently for each coordinate.
Then writing $\sin{\theta_{\xi}}$ and $-\cos{\theta_{\xi}}$ as a Fourier series and combining it with those of $\hat{\gamma}(\theta_{\xi})$ we can evaluate the inverse Fourier transform in polar coordinates, see Appendix~\ref{sec:appendix:spatial:2d} for details.
%\begin{align}
%  e^{i \langle x , \xi \rangle} = \sum_{m \in \Z} i^m \, e^{i m (\theta_x - \theta_{\xi}} \, J_m( \vert \xi \vert , \vert x \vert)
%\end{align}
%where $J_m$ is the Bessel function of order $m$.
This yields
\begin{align}
  \label{eq:psi:divfree:2d:space}
	\vec{\psi}(x) &= \frac{1}{2}
    \sum_{\sigma \in \pm 1} \sum_{m} i^{m + \sigma} \, \beta_m  \, e^{i (m + \sigma) \theta_x}  h_{m + \sigma}(\vert x \vert)
  \begin{pmatrix}
    \textrm{-}\sigma
    \\
    i
  \end{pmatrix}
\end{align}
where the $h_{m + \sigma}(\vert x \vert)$ are the inverse Hankel transforms of $\hat{h}(\vert \xi \vert)$.
For the Simoncelli window~\cite{Portilla2000} these also have closed form expressions, which are available in the reference implementation.

Eq.~\ref{eq:psi:divfree:2d:space} defines a family of wavelet functions that is by construction divergence free and  whose angular localization can be controlled using the $\beta_m$, see Fig.~\ref{fig:psis:2d} for examples.
We will return to suitable choices of the angular localization at the end of the section.
In the special case when $\hat{\gamma}(\theta_{\xi})$ is isotropic, i.e. $\beta_m = \delta_{0m}$, one obtains $\vec{\psi}(x) = \hat{h}_1(\vert x \vert) \, \vec{e}_{\theta_x}$.
This is an isotropic, divergence free vector field in space that can be interpreted as an isolated vortex, see Fig.~\ref{fig:psis:2d}, left.

\begin{figure}[t]
  \begin{center}
  \includegraphics[width=0.24\textwidth]{psihat_ns_j3_ko6}
  \includegraphics[width=0.24\textwidth]{psihat_ns_j3_ko5}
  \includegraphics[width=0.24\textwidth]{psihat_ns_j3_ko4}
  \includegraphics[width=0.24\textwidth]{psihat_ns_j3_ko3}
  \includegraphics[width=0.24\textwidth]{psi_ns_j3_ko6}
  \includegraphics[width=0.24\textwidth]{psi_ns_j3_ko5}
  \includegraphics[width=0.24\textwidth]{psi_ns_j3_ko4}
  \includegraphics[width=0.24\textwidth]{psi_ns_j3_ko3}
  \end{center}
  \caption{Different orientations for directional wavelets for $j=3$ in the frequency (top) and spatial (bottom) domains. As shown in Sec~\ref{sec:construction:2d:directional} and Sec.~\ref{sec:experiments}, significant coefficients are only obtained when a flow has anisotropic structures aligned with the wavelet.}
  \label{fig:psis:ns:2d:ko}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Properties of wavelets}

A critical property of the wavelet defined in Eq.~\ref{eq:psi:divfree:2d:frequency} is that these generate a Parseval tight frame for the space $L_2^{\textrm{div}}(\mathbb{R}^{2,2})$ of divergence free vector fields with finite $L_2$-norm.
Hence, most of the conveniences of an orthonormal basis are available and in particular primary and dual frame functions coincide and Parseval's identity holds so that the norm of the expansion coefficients equals those of the signal.
See for example Daubechies classical treatise~\cite[Ch. 3]{Daubechies1992} or the expository articles by Kovacevic and Chebira~\cite{Kovacevic2007,Kovacevic2007a} for more details on frames.

\begin{proposition}
    \label{prop:polarlet:2d:parseval}
    Let $U_j$ be the $(M_j \times 2 N_j + 1)$-dimensional matrix formed by the angular localization coefficients $\beta_{n}^{j,t} = \beta_{n}^{j} \, e^{-i n t (2\pi / M_{j})}$ for the $M_j$ different orientations, and let $D_j$ be a diagonal matrix of size $(2 N_j + 1) \times (2 N_j + 1)$.
  When the Cald{\`e}ron admissibility condition $\sum_{j \in \mathbb{Z}} \big\vert \hat{h}( 2^{-j} \vert \xi \vert ) \big\vert^2 = 1$, $\forall \xi \in \mathbb{R}^2$ is satisfied and $U_j^H U_j = D_j$ with $\mathrm{tr}( D_j ) = 1$ for all levels $j$,
  then any divergence free vector field $\vec{u}(x) \in L_2^{\mathrm{div}}(\mathbb{R}^{2,2})$ has the representation
  \begin{subequations}
  \begin{align}
    \label{eq:polarlet:2d:parseval}
    \vec{u}(x) = \sum_{j \in \mathbb{Z}} \sum_{k \in \mathbb{Z}^2} \sum_{t=1}^{M_j} \big\langle \vec{u}(y) , \vec{\psi}_{j,k,t}(y) \big\rangle \, \vec{\psi}_{j,k,t}(x)
  \end{align}
  with frame functions
  \begin{align}
    \vec{\psi}_{j,k,t}(x) = \frac{2^j}{2\pi} \, \vec{\psi}\big( R_{2\pi t / M_j} (2^j x - k) \big)
  \end{align}
  \end{subequations}
  where $\vec{\psi}(x)$ is given by Eq.~\ref{eq:psi:divfree:2d:space} and $R_{2\pi t / M_j}$ is the rotation by $2\pi t / M_j$.
\end{proposition}

\begin{proof}
Taking the Fourier transform of Eq.~\ref{eq:polarlet:2d:parseval}, using Parseval's theorem, and with Eq.~\ref{eq:psi:divfree:2d:frequency} one obtains
\begin{subequations}
\begin{align}
    \hat{u}(\xi) \, \vec{e}_{\theta}
    &= \sum_{j \in \mathbb{Z}} \sum_{k \in \mathbb{Z}^2} \sum_{t=1}^{M_j} \Big\langle \hat{u}(\eta) \, \vec{e}_{\theta} , \hat{\psi}_{j,k,t}(\eta) \, \vec{e}_{\theta} \Big\rangle \, \hat{\psi}_{j,k,t}(\xi) \, \vec{e}_{\theta}
    \\
    \label{prop:polarlet:2d:parseval:2}
    &= \underbrace{\sum_{j \in \mathbb{Z}} \sum_{k \in \mathbb{Z}^2} \sum_{t=1}^{M_j} \Big\langle \hat{u}(\eta) , \hat{\psi}_{j,k,t}(\eta) \Big\rangle \, \hat{\psi}_{j,k,t}(\xi)}_{\textrm{scalar polar wavelet expansion of $\hat{u}(\xi)$}} \, \vec{e}_{\theta}
\end{align}
\end{subequations}
with the inner product in the second line now being those for scalar functions and $\hat{\vec{u}}(\eta) = \hat{u}(\eta) \, \vec{e}_{\theta}$ for some scalar $\hat{u}(\eta)$ by the divergence freedom of $\vec{u}(x)$.
In Eq.~\ref{prop:polarlet:2d:parseval:2}, $\vec{e}_{\theta}$ is fixed and the other terms provide a scalar polar wavelet expansion of the scalar magnitude function $\hat{u}(\xi)$.
Since the proposition uses the same assumptions required for scalar polar wavelets to form a Parseval tight frame, see~\cite[Proposition 4.1]{Unser2013} for the isotropic case and~\cite[Proposition 4.2]{Unser2013} for the anisotropic one, the result follows.
%A complete proof is provided in the supplementary material.
\end{proof}

As usual, in practice one uses scaling functions $\phi_s(x)$ for a signal's low frequency part and a variation of Proposition~\ref{prop:polarlet:2d:parseval} holds in this case.
Next to being Parseval tight, our divergence free wavelets satisfy other useful properties:
\begin{enumerate}
  \item \emph{Intuitive correspondence:} The isotropic frame functions can be interpreted as isolated vortices and the directional wavelets are similar to flows along boundaries.
  \item \emph{Ideal divergence freedom:} Our wavelets are divergence free in the ideal, analytic sense and, with $\hat{h}(\vert \xi \vert)$ from~\cite{Portilla2000}, which yields a closed form expression for the radial windows $h_m(\vert x \vert)$ in the spatial domain, they can be evaluated to arbitrary precision.
%  \item \emph{Vanishing moments:} When $\hat{h}( \vert \xi \vert)$ has vanishing moments then so has the isotropic divergence free wavelet $\vec{\psi}(x)$.
%  \item \emph{Steerability:} For fixed $j$, when the $\beta_n^{j,t}$ generate a frame for $\mathcal{H}_{j}(S^1)$, the Fourier series space for which the $\beta_m^{j,t}$ are non-zero as a function of $m$, our wavelets are steerable.
%    % For typical angular window functions the frame condition is satisfied since Eq.~\ref{eq:admissibility:calderon:angular} with $D_j = \mathrm{Id}$ is the perfect reconstruction condition for frames and hence a convenient choice for the $\beta_n^{j_s,t_s}$ are those corresponding to a frame.
  \item \emph{Analytic, polar frequency representation:} The analytic, polar separable construction of $\smash{\hat{\vec{\psi}}(\xi)}$ enables the closed form computation of differential operators such as curl, i.e. the vorticity of the fluid velocity vector field.
      %This is beneficial for example for Galerkin projection or when the curl has physical significance.
  \item \emph{Closed form spatial representation:} The wavelets have closed form expressions in the spatial domain, which are useful for example for reconstruction and interpolation~\cite{Lessig2018a} and to compute advection.
  \item \emph{Multi-resolution structure and fast transform:} The multi-resolution structure and associated fast transform of our wavelets enable efficient analysis and reconstruction.
\end{enumerate}

\begin{figure}
  \includegraphics[trim={80 100 30 20},clip,width=0.32\textwidth]{psidiv3d_hat_j0.pdf}
  \includegraphics[trim={80 100 30 20},clip,width=0.32\textwidth]{psidiv3d_hat_j2.pdf}
  \includegraphics[trim={80 100 30 20},clip,width=0.32\textwidth]{psidiv3d_hat_j3.pdf}
  \includegraphics[trim={80 100 30 20},clip,width=0.32\textwidth]{psidiv3d_j0.pdf}
  \includegraphics[trim={80 100 30 20},clip,width=0.32\textwidth]{psidiv3d_j2.pdf}
  \includegraphics[trim={80 100 30 20},clip,width=0.32\textwidth]{psidiv3d_j3.pdf}
  \caption{Divergence free wavelets in three dimensions, top row in the frequency domain and bottom row in the spatial one. The left function is isotropic around the $x_3$ axis and the other ones are directional modeling a high frequency feature across the $x_1$-$x_2$ plane.}
  \label{fig:psis:3d}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Directional Wavelets}
\label{sec:construction:2d:directional}

The angular window $\hat{\gamma}(\theta)$, which is defined through the Fourier series coefficients $\beta_m^j$, provides directional localization in the Fourier domain.
By Eq.~\ref{eq:psi:divfree:2d:space}, the directionality is preserved by the inverse Fourier transform and the wavelets in the spatial domain have the same angular selectivity.
In the scalar theory, such a directional localization was first introduced for steerable wavelets~\cite{Simoncelli1995,Perona1991} to detect oriented features and it is also critical for the efficient approximation of discontinuous signals using curvelets and similar constructions~\cite{Candes1999a,Candes2005a,Labate2005,Do2005a}.
See Fig.~\ref{fig:wf} for some intuition.
%Conceptually, the connection between directionality and the efficient analysis and representation of high-frequency features is the fact that the (localized) Fourier transform of a (smoothed) discontinuity decays slowly only along the direction of the normal $\vec{n}$ in the Fourier domain, i.e. when $\xi \approx \vec{n}$, see~\cite[Ch. XIV]{Stein1993} or~\cite[Vol. 1, Ch. VIII]{Hoermander2004} for precise statement about localization and~\cite[Sec. 5]{Candes2005a} for the case when one has a smoothed discontinuity.
%%In the simplest case, the signal $f(x)$ is unity for $x_2 < 0$ and zero otherwise with normal along the $x_2$-axis.
%%Then $\hat{f}(\xi) = \delta(\xi_1) \, 1  $ with $1/ \vert \xi_2 \vert$ decay along the $\xi_2$ axis.
%Hence, when $\hat{\gamma}(\theta)$ is oriented so that it is centered around the normal direction $\vec{n}$ of the discontinuity then one obtains a large frame coefficients while when it has a very different orientation then the coefficient is negligible because the window and the discontinuity have essentially disjoint support in frequency space, see Fig.~\ref{fig:psis:ns:2d:ko}.

For divergence free vector fields, our directional, divergence free wavelets yield analogous behavior than steerable wavelets and curvelets in the scalar setting.
This can be seen by computing the frame coefficient $u_s$ for a fluid vector field $\vec{u}(x)$, i.e.
\begin{subequations}
\begin{align}
    u_s = \big\langle \vec{u}(x) , \vec{\psi}_s(x) \big\rangle
  &= \Big\langle \hat{\vec{u}}(\xi) , \hat{\vec{\psi}}_s(\xi) \Big\rangle .
\end{align}
Since both $\vec{u}(x)$ and $\vec{\psi}_s(x)$ are divergence free, and hence tangential to $S_{\vert \xi \vert}^1$, they both have $\vec{e}_{\theta_{\xi}}$ as vector component.
Using that $\vec{e}_{\theta_{\xi}}$ is a unit vector one obtains
\begin{align}
  \label{eq:2d:approx:curvelets:2}
  u_s
  &= \big\langle \hat{u}(\xi) \, \vec{e}_{\theta_{\xi}} \, , \, -i \, \hat{\gamma}(\theta_{\xi}) \, \hat{h}(\vert \xi \vert) \, \vec{e}_{\theta_{\xi}} \big\rangle
  \\[3pt]
  &= \big\langle \hat{u}(\xi) \, , \, -i \, \hat{\gamma}(\theta_{\xi}) \, \hat{h}(\vert \xi \vert)  \big\rangle
\end{align}
\end{subequations}
with the inner product in the second line again being those for scalar functions.
%Since a divergence free vector field in $\R^2$ behaves in the Fourier domain like a scalar function (it consists of a scalar magnitude function $\hat{u}(\xi)$ and a fixed vector field), o
%Our directional, divergence free wavelets detect oriented features in a flow, e.g. the behavior in the vicinity of a boundary or the wake behind an object.
Thus, our directional, divergence free wavelets detect oriented features in a flow, i.e. where the scalar magnitude function $\hat{u}(\xi)$ decays slowly.
We will numerically validate this in Sec.~\ref{sec:experiments}.

\begin{figure}
  \includegraphics[width=0.8\textwidth]{wf.pdf}
  \caption{\emph{Left:} Discontinuous, scalar signal $f(x)$ with normal pointing towards $(1,1)$ around the origin. The ellipses indicate directional wavelets aligned (red) and unaligned (cyan) with the discontinuity. \emph{Right:} Conceptual view of the localized Fourier transform $\widehat{f \phi}$. It decays slowly only along the directions $\bar{\xi} \approx \vec{n}$. Hence, a wavelet $\hat{\psi}(\xi)$ supported sufficiently far from the origin will overlap $\widehat{f \phi}$ only when its orientation is aligned with the direction of slow decay, and hence with the normal of the discontinuity.
    We refer to~\cite[Ch. XIV]{Stein1993} and~\cite[Vol. 1, Ch. VIII]{Hoermander2004} for precise statements about the local Fourier transform of discontinuous signals and to~\cite{Candes2005a} for their approximation using wavelet-like functions.}
  \label{fig:wf}
\end{figure}


Interestingly, in the vector-valued case one has an additional degree of freedom not present in the scalar setting.
For real-valued signals, the Fourier transform is symmetric around the origin and hence $\vec{e}_{\theta_{\xi}}$ can point either in the same or opposite directions in the two half-spaces, see the last two columns in Fig.~\ref{fig:psis:2d}, top.
The two choices yield starkly different spatial wavelets $\vec{\psi}_s(x)$: when $\vec{e}_{\theta_{\xi}}$ points in opposite directions one obtains a shear-like behavior while a consistent direction of $\vec{e}_{\theta_{\xi}}$ yields a localized uni-directional streaming-like flow, see again the two rightmost columns in Fig.~\ref{fig:psis:2d}.
Directional wavelets corresponding to the two behaviors are conveniently modeled using Fourier series coefficients $\beta_m$ that are nonzero only for even $m$, which yields shear-like flows, or nonzero only for odd $m$, for streaming-like flows, see Fig.~\ref{fig:beta_m}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Divergence free polar wavelets in 3D}
\label{sec:construction:3d}

To carry the foregoing construction over to three dimensions, we need an equivalent of the tangent vector $\vec{e}_{\theta_{\xi}}$, which was the crucial ingredient ensuring divergence freedom in $\mathbb{R}_x^2$.
By the Hedgehog theorem, however, any smoothly changing basis tangential to the sphere will become singular at some point on $S^2$.
We escape the theorem with the following construction.

\begin{proposition}
  Let $\vec{\tau}_a$ be the tangent vector field of $S^2$ induced by the longitudal geographic coordinate $\phi_a$ with respect to the $a^{\textrm{th}}$ axis, i.e. $\vec{\tau}_a = \partial / \partial \phi_a$.
  Then for every $\omega \in S^2$ the set
  \begin{align}
    H(\omega) = \big\{ \vec{\tau}_1(\omega) , \, \vec{\tau}_2(\omega) , \, \vec{\tau}_3(\omega) \big\}
  \end{align}
  forms a Parseval tight frame for $T_{\omega} S^2$.
  We will refer to $H$ as the Hedgehog frame.
\end{proposition}

The proposition can be checked by an explicit calculation and, in a more general form, can also be found in~\cite{Freeman2014}.
Intuitively, it holds because the three vectors compensate each other, e.g. $\vec{\tau}_3$ vanishes at the North pole but this is exactly where $\vec{\tau}_1$ and $\vec{\tau}_2$ form an orthonormal basis.


\begin{figure}
  \includegraphics[width=\textwidth]{beta_m.pdf}
  \caption{Examples for coefficients $\beta_m$ that define the angular localization windows $\hat{\gamma}(\theta_{\xi})$. Functions yielding a shear-like flow have $\beta_m$ that are non-zero only for even $m$ (blue) while those yielding a streaming-like flow behavior have nonzero $\beta_m$ only for odd $m$ (yellow).}
  \label{fig:beta_m}
\end{figure}

With the Hedgehog frame, we can proceed as before to construct a divergence free wavelet frame: we choose a vectorial part that is inherently tangential to the frequency sphere, namely $\vec{\tau}_a$, and obtain angular localization with a scalar window function.
Our mother wavelets are thus defined as
\begin{align}
  \label{eq:wavelets:3d:frequency}
  \hat{\vec{\psi}}_a(\xi)
  = \hat{\psi}_a(\xi) \, \vec{\tau}_a
  = -i \, \left( \sum_{l=0}^L \sum_{m=-l}^l \kappa_{lm} \, y_{lm}(\bar{\xi}) \right) \hat{h}( \vert \xi \vert) \, \vec{\tau}_a
\end{align}
with now one for each coordinate axis.
By expanding $\vec{\tau}_a$ into spherical harmonics, the spatial representation $\vec{\psi}_a(\xi)$ can be computed in closed form using a calculation analogous to those in two dimensions, see Appendix~\ref{sec:appendix:spatial:3d} for details.
It is given by
\begin{align}
  \label{eq:wavelets:3d:general}
  \vec{\psi}_3(x) =
  \frac{2}{\sqrt{3}} \sum_{l,m} & \, \kappa_{lm}
   \sum_{l_2=l-1}^{l+1} i^{l_2} \,  h_{l_2}( \vert x \vert)
  \sum_{\sigma \in \pm 1}  G_{l m;1 \sigma}^{l_2,m+\sigma} \, y_{l_2,m+\sigma}(\bar{x})
  \begin{pmatrix}
    -1
    \\[-1pt]
    i \, \sigma
    \\[-1pt]
    0
  \end{pmatrix}
\end{align}
and analogously for the other two coordinate axes.
Here the $G_{l m;1 \sigma}^{l_2,m+\sigma}$ are spherical harmonics product coefficients, see Appendix~\ref{sec:preliminaries:sh}.
We also again have that the spatial representation of an isotropic wavelet $\smash{\hat{\vec{\psi}}_a(\xi)} = \hat{h}( \vert \xi \vert) \, \vec{\tau}_a$ is isotropic in space, i.e. $\vec{\psi}_a(x) = -\sqrt{2 / \pi} \, h_1 \big(\vert x \vert\big) \, \vec{\tau}_a$, with isotropy now around the $a^{\textrm{th}}$ axis.
%\begin{align}
%  \vec{\psi}_i^{\textrm{iso}}(x) = -\sqrt{\frac{2}{\pi}} \, h_1 \big(\vert x \vert\big) \, \vec{\tau}_i .
%\end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Properties of wavelets}
As in the scalar case, under suitable admissibility conditions the just defined wavelets form a Parseval tight frame for the space $L_2^{\textrm{div}}(\mathbb{R}^{3,3})$ of divergence free vector fields in $\R^3$ with finite $L_2$-norm.

\begin{proposition}
  \label{prop:tight_frame:3d}
  Let $w_{j,t}$ be the $(L_j+1)^2$-dimensional vector formed by the rotated angular localization coefficients $\kappa_{lm}^{j,t} = \sum_{m' = -l}^l W(\lambda_t)_{l,m}^{m'} \kappa_{l,m'}$ for a localization window centered at $\lambda_t$, where $W(\lambda_t)_{l,m}^m$ is the Wigner-D matrix implementing rotation in the spherical harmonics domain, and let $G^{lm}$ be the $(L_j+1)^2 \times (L_j+1)^2$ dimensional matrix formed by the spherical harmonics product coefficients for fixed $(l,m)$.
  When the Cald{\`e}ron condition $\sum_{j \in \mathbb{Z}} \big\vert \hat{h}( 2^{-j} \vert \xi \vert ) \big\vert^2 = 1$, $\forall \xi \in \mathbb{R}^3$ is satisfied and $\delta_{l,0} \delta_{m,0} = \sum_{t=0}^{M_j} w_{j,t} \, G^{lm} \, w_{j,t}$ (where $\delta_{i,j}$ is the Kronecker delta) then any $\vec{u}(x) \in L_2^{\textrm{div}}(\mathbb{R}^{3,3})$ has the representation
  \begin{subequations}
  \begin{align}
    \label{eq:tight_frame:3d}
    \vec{u}(x) = \sum_{a=1}^3 \sum_{j \in \mathbb{Z}} \sum_{k \in \mathbb{Z}^3} \sum_{t=1}^{M_j} \big\langle \vec{u}(y) , \vec{\psi}_{j,k,t}^a(y) \big\rangle \, \vec{\psi}_{j,k,t}^a(x)
  \end{align}
  with frame functions
  \begin{align}
    \vec{\psi}_{j,k,t}^a(x) = \frac{2^{3j/2}}{(2\pi)^{3/2}} \, \vec{\psi}_a \big( R_{\lambda_t} (2^{j} x -  k ) \big) ,
  \end{align}
  \end{subequations}
  for $\vec{\psi}_a(x)$ defined in Eq.~\ref{eq:wavelets:3d:general} and $R_{\lambda_t}$ the rotation from the North pole to $\lambda_t$.

%  \begin{align}
%    \sum_{j \in \mathbb{Z}} \big\vert \hat{h}( 2^{-j} \vert \xi \vert ) \big\vert^2 \quad , \quad \forall \xi \in \mathbb{R}^3
%  \end{align}
%  and the $(L_j+1)^2$-dimensional vector $u_{j,t}$ formed by the $\kappa_{lm}^{j,t}$ for fixed $j$, $t$ satisfies
%  \begin{align}
%    \label{eq:admissibility:calderon:angular:3d}
%    \delta_{l,0} \delta_{m,0} = \sum_{t=0}^{M_j} u_{j,t} \, G^{lm} \, u_{j,t} .
%  \end{align}
\end{proposition}

\begin{proof}
Taking the Fourier transform of Eq.~\ref{eq:tight_frame:3d}, using Parseval's theorem, and with Eq.~\ref{eq:wavelets:3d:frequency} we obtain
\begin{subequations}
\begin{align}
  \hat{\vec{u}}(x)
  &= \sum_{a=1}^3 \sum_{j \in \mathbb{Z}} \sum_{k \in \mathbb{Z}^3} \sum_{t=1}^{M_j} \Big\langle \hat{\vec{u}}(\eta) \, , \, \hat{\psi}_{j,k,t}(\eta) \, \vec{\tau}_a(\eta) \Big\rangle \, \hat{\psi}_{j,k,t}^a(\xi) \, \vec{\tau}_a(\xi)
  \\
   &= \sum_{a=1}^3 \underbrace{\sum_{j \in \mathbb{Z}} \sum_{k \in \mathbb{Z}^3} \sum_{t=1}^{M_j} \Big\langle \hat{u}_a(\eta) \, , \, \hat{\psi}_{jkt}(\eta) \Big\rangle \, \hat{\psi}_{jkt}^a(\xi)}_{\textrm{scalar polar wavelet frame for $\hat{u}_a(\eta)$}} \, \vec{\tau}_a(\xi) .
\end{align}
\end{subequations}
Here $\hat{u}_a(\eta) = \hat{\vec{u}}(\eta) \cdot \vec{\tau}_a(\eta)$, i.e. the pointwise projection of the vector $\hat{u}_a(\eta)$ onto the Hedgehog frame vector $\vec{\tau}_a(\eta)$ at $\eta$, so that $\hat{\vec{u}}(\eta) = \sum_a \hat{u}_a(\eta) \, \vec{\tau}_a(\eta)$ by the tight frame property of the $\vec{\tau}_a$.
For the coordinate function $\hat{u}_a(\xi)$ one has a scalar polar wavelet frame expansion.
Since the proposition uses the same conditions that are required for scalar polar wavelets in $\R^3$ to form a Parseval tight frame, the result follows from the existing proofs for the scalar case.
See~\cite[Proposition 4.1]{Ward2014} for the isotropic result and~\cite[Theorem 2.4]{Ward2014} for those for the anisotropic case.
%See the supplementary material for a detailed proof.
\end{proof}

The three dimensional divergence free wavelets have the same useful properties we already observed in two dimensions, in particular they are divergence free in an ideal, analytic sense, they have closed form expressions in frequency and space, a multi-resolution structure and fast transforms.
%, and an intuitive correspondence to natural flow phenomena, see Fig.~\ref{fig:psis:3d}.


\begin{figure}[t]
  \includegraphics[width=0.1725\textwidth]{polarlets_divfree_sig_ref_with_legend.pdf}
  \includegraphics[width=0.155\textwidth]{polarlets_divfree_sig_rec_j-1.pdf}
  \includegraphics[width=0.155\textwidth]{polarlets_divfree_sig_rec_j0.pdf}
  \includegraphics[width=0.155\textwidth]{polarlets_divfree_sig_rec_j1.pdf}
  \includegraphics[width=0.155\textwidth]{polarlets_divfree_sig_rec_j2.pdf}
  \includegraphics[width=0.155\textwidth]{polarlets_divfree_sig_rec_j3.pdf}
  \\
  \includegraphics[width=0.1725\textwidth]{polarlets_divfree_sig_ref_with_legend_placeholder.png}
  \includegraphics[width=0.155\textwidth]{polarlets_divfree_sig_rec_err_j-1.pdf}
  \includegraphics[width=0.155\textwidth]{polarlets_divfree_sig_rec_err_j0.pdf}
  \includegraphics[width=0.155\textwidth]{polarlets_divfree_sig_rec_err_j1.pdf}
  \includegraphics[width=0.155\textwidth]{polarlets_divfree_sig_rec_err_j2.pdf}
  \includegraphics[width=0.155\textwidth]{polarlets_divfree_sig_rec_err_j3.pdf}
  \caption{Level-by-level reconstruction of a divergence free fluid vector field (top left) with free slip boundary conditions with only isotropic basis functions from $j=-1$ (second column from left), i.e using only scaling functions, to $j=3$ (right). The second row shows the error in the reconstructed vector field. For $j=3$ the vector field is well represented except close to the boundaries where one still has a relatively large error since, firstly, the number of levels is too small to fully resolve the signal and, secondly, the apron region around the flow domain is relatively small.
  With anisotropic functions the error can be substantially reduced, see Fig.~\ref{fig:sig:boundary}.}
  \label{fig:rec_err_sig}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Fast Transform}
\label{sec:div_free:fast_transform}

The fast wavelet transform provides an efficient means to obtain the wavelet coefficients of a signal, in our case a fluid velocity vector field, without the need to use numerical quadrature.
It proceeds by splitting the signal $f_{j+1}$ at scale $j+1$ into a low frequency part $f_j$ on level $j$, represented by scaling function coefficients, and a high frequency part, represented by wavelet coefficients.
By linearity it suffices to determine the projection for the basis functions, which are described by the filter taps
\begin{subequations}
\begin{align}
  \alpha_{j,k} &= \left\langle \vec{\phi}_{j,0}(x) , \vec{\phi}_{j+1,k}(x) \right\rangle
  \\[5pt]
  \beta_{j,k,t} &= \left\langle \vec{\psi}_{j,0,t}(x) , \vec{\phi}_{j+1,k}(x) \right\rangle
  \\[5pt]
  \gamma_{j,k,t,t'} &= \left\langle \vec{\psi}_{j,0,t}(x) , \vec{\psi}_{j+1,k,t'}(x) \right\rangle
  \\[5pt]
  \delta_{j,k,t} &= \left\langle \vec{\psi}_{j,0,t}(x) , \vec{\phi}_{j,k}(x) \right\rangle
\end{align}
\end{subequations}
with the $\gamma_{j,k,t,t'}$ only necessary for analysis, i.e. projecting a signal into the wavelet basis, and $\delta_{j,k,t}$ only for the reconstruction, see Appendix~\ref{sec:appendix:fast_transform} for details.
Our construction enables the computation of the filter taps in closed form, avoiding expensive numerical quadrature and ensuring that they can be obtained to any required accuracy.

%For notational simplicity we will suppress the dependence on the orientation in this section.
Without loss of generality, we will consider the calculation for the $\beta_{j,k}$ in two dimensions.
Using Parseval's theorem we obtain
\begin{subequations}
\begin{align}
  \beta_{j,k} = \left\langle \hat{\vec{\psi}}_{j,0}(\xi)  \, ,  \, \hat{\vec{\phi}}_{j,k+1}(\xi) \right\rangle
\end{align}
and since both $\hat{\vec{\psi}}_{j,0}(\xi)$ and $\hat{\vec{\phi}}_{j,k+1}(\xi)$ have the same vectorial part, namely $\vec{e}_{\theta}$, this reduces to
\begin{align}
  \beta_{j,k} = \left\langle \hat{\psi}_{j,0}(\xi)  \, ,  \, \hat{\phi}_{j,k+1}(\xi) \right\rangle .
\end{align}
where the inner product is now those for scalar functions and the filter taps computation is the same as for scalar polar wavelets~\cite{Lessig2018a}.
In particular, expanding $\hat{\psi}_{j,0}(\xi)$ and $\hat{\phi}_{j,k+1}(\xi)$ using their definitions one obtains
\begin{align}
  \label{eq:fast_transform:beta}
  \beta_{j,k}
  &= 2\pi \sum_{n} i^n \, \beta_n \, \int_{\R_{\vert \xi \vert}^+} \hat{h}(2^{-j} \vert \xi \vert) \, \hat{g}(2^{-j+1} \vert \xi \vert) \, J_m(\vert \xi \vert \, \vert k \vert) \, \vert \xi \vert \, d\vert \xi \vert
  \\[5pt]
  &= 2\pi \sum_{n} i^n \, \beta_n \, B_{j}(k)
\end{align}
\end{subequations}
with $B_{j}(k)$ having a closed form expression and being scale invariant, see the reference implementation.
Hence, the $\beta_{j,k}$ can be evaluated using a finite computation and to any required accuracy.
An analogous calculation applies to the $\alpha_{j,k}$, $\gamma_{j,k,t,t'}$ and $\delta_{j,k,t}$.
In three dimensions, the tightness of the Hedgehog frame allows a similar reduction of the vector-valued case to the computation of filter taps for scalar polar wavelets.

Since our wavelets do not have compact support in space, the fast transform requires formally infinite sums.
They become finite in the finite precision available on practical computers but the filters still have a very large number of taps.
One thus typically truncates the filters, which, however, also results in reduced accuracy.
A computation of the frame coefficients in the frequency domain based on the FFT can hence be more accurate and efficient than the fast transform.
See again Appendix~\ref{sec:appendix:fast_transform} for a more detailed discussion.


==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\begin{figure}
  \begin{center}
  \includegraphics[width=0.65\columnwidth]{polarlets_divfree_sig_err_rec.pdf}
  \end{center}
  \caption{$L_{2}$ (yellow) and $L_{\infty}$ error rates for the level-by-level reconstruction shown in Fig.~\ref{fig:rec_err_sig}.}
  \label{fig:rec_err_sig:errrates}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation of wavelets}
\label{sec:experiments:implementation}

We developed a reference implementation of our divergence free polar wavelets in Mathematica.\footnote{\url{http://graphics.cs.uni-magdeburg.de/projects/psidiv/mathematica.zip}}
For the radial window function we used the Portilla-Simoncelli window~\cite{Portilla2000}, which yields closed form expressions for the wavelets in the spatial domain~\cite{Lessig2018a}.
In two dimensions, the angular window functions $\hat{\gamma}(\theta)$ are an extension of those used in~\cite{Lessig2018a} which are based on the wavelets for the circle developed by Walter and Cai~\cite{Walter1999}, see Fig.~\ref{fig:beta_m}.
Since for the two different types of directional wavelets only even and odd Fourier series coefficients are nonzero, respectively, they can be combined without interference and it is straight forward to construct a tight frame containing both types of boundary functions.
%For the no-slip boundary wavelets only the even coefficients are non-zero while for the free-slip ones only the coefficients for odd $m$ are non-zero and these are purely imaginary to obtain real-valued wavelets in the spatial domain.
In three dimensions, the angular windows are those from~\cite{McEwen2016} for wavelets on the sphere and the orientations, which are non-trivial because on $S^2$ one has no equivalent of a uniform grid, are a custom construction ensuring that the discrete spherical wavelets form a tight frame and satisfy the requirements in Proposition~\ref{prop:tight_frame:3d}~\cite{Lessig2018a}.

\begin{figure}
  \includegraphics[width=0.32\columnwidth]{polarlets_divfree_sig_err_field_iso.pdf}
  \includegraphics[width=0.32\columnwidth]{polarlets_divfree_sig_err_field_full.pdf}
  \includegraphics[width=0.32\columnwidth]{polarlets_divfree_sig_err_field_sparse.pdf}
  \caption{Reconstruction error for the fluid velocity vector field in Fig.~\ref{fig:rec_err_sig} with different functions on the finest level $j=3$: only isotropic functions (left), with all directional functions (middle), with only the directional functions aligned with the boundary (right). The middle and right plot differ only slightly. One can hence predict the sparsity, i.e. the non-negligible frame coefficients, when the boundary orientation is known and does not have to compute all of them.}
  \label{fig:sig:boundary}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Analysis of fluid velocity vector fields}
\label{sec:experiments:analysis}

In our experiments we considered two fluid velocity vector fields, one that is divergence free in the analytic sense, see Fig.~\ref{fig:rec_err_sig}, and a classical flow around a ball obtained with an FEM simulation that is approximately divergence free, see Fig.~\ref{fig:ball}.

The ideal divergence free flow was obtained as a linear combination of divergence free eigenfunctions of the vector-Laplacian for the square.
In the experiment we first studied the approximation power with only isotropic functions.
Fig.~\ref{fig:rec_err_sig} shows that with four levels the velocity vector field is already well resolved except around the boundaries of the domain.
There the vector field is discontinuous (when considered in $\R^2$) and the small number of levels is not sufficient to fully resolve the signal.
Additionally, the apron region around the flow domain is relatively small.
To reduce the latter effect, we also studied the approximation with anisotropic functions on the finest level.
Fig.~\ref{fig:sig:boundary} shows that the use of directional wavelets approximately halves the error.
The $L_2$ and $L_{\infty}$ error rates for the experiment as a function of the level and with and without directional wavelets on the finest level are provided in Fig.~\ref{fig:rec_err_sig:errrates}.

For the flow around the ball we studied the sparsity and the potential of the wavelets to detect specific flow features.
The coefficient plots in Fig.~\ref{fig:ball} demonstrate that our directional wavelets provide good angular selectivity and yield a correspondingly high sparsity.
They also demonstrate that directional wavelets are not only useful for modeling boundaries but also for other highly anisotropic features such as a von K{\'a}rm{\'a}n vortex street.


==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Turbulent fluids exhibit features at many different scales with fine details often being localized to small neighborhoods.
% , often with a high degree of spatial localization.
% with highly turbulent regions often having a high spatial localization.
An efficient analysis and representation of fluid velocity vector fields hence has to adapt to these multiple scales and exploit their locality.
For incompressible fluids, it also should respect the divergence free nature of the vector field.
%Infinitesimally, they are described by divergence free vector fields.
%Their efficient and faithful representation is hence of great importance in manifold fields, ranging from the basic sciences~\cite{Federbush1986,Federbush1987} to applied areas such as medical imaging~\cite{Bostan2015}.
% to antenna design~\cite{Galvan2017} and medical

In this work, we present a vector-valued wavelet frame for the analysis and representation of incompressible fluids.
%for the efficient and faithful representation of such vector fields that has many expedient properties.
% that is numerically practical and expedient through a simple yet judicious mathematical construction.
Our wavelets form a Parseval tight frame, are divergence free in the ideal, analytic sense, have an intuitive correspondence to vortices, closed form expressions in frequency and space, an associated multi-resolution structure, and fast transforms with filter taps that can be computed in closed form.
Furthermore, and in contrast to existing work, our construction also allows for well-defined angular selectivity, ranging from isotropic functions that can be interpreted as classical vortices to angularly highly selective, divergence free wavelets that provide a vector-valued analogue of curvelets.
 As we demonstrate, the directional wavelets are well suited to model divergence free vector fields in the vicinity of boundaries and around highly anisotropic features like those occurring in the wake behind an object.
%These properties make our wavelets well suited for the efficient analysis and representation of incompressible fluid flows and enable us to resolve the different scales that occur.

% The expedient properties of our wavelets are enabled by respecting the intrinsic structure of divergence free vector fields.
The expedient properties of our wavelets result from a construction that exploits the intrinsic structure of divergence free vector fields in the Fourier domain, namely that the Fourier transform $\hat{\vec{u}}(\xi)$ is tangential to the sphere
\setlength{\columnsep}{4pt}
\begin{wrapfigure}[11]{r}[0pt]{0.4\columnwidth}
  \centering
  \vspace{-11pt}
  \includegraphics[width=0.4\columnwidth]{conceptual}
  \vspace{-10pt}
\end{wrapfigure}
%We exploit that divergence freedom is a simple geometric condition in the Fourier domain:
$\smash{S_{\xi}^{d-1}}$ in frequency space $\mathbb{R}_{\xi}^d$, see the inset figure.
% Consequently, divergence free basis functions are naturally defined in spherical (or polar) coordinates where $\smash{\vec{\xi} \cdot \hat{\vec{u}}(\xi) = 0}$ can be ensured by choosing a vector field without radial component.
% We hence define the scalar window functions of our wavelets $\smash{\hat{\vec{\psi}}(\xi)}$ in spherical (or polar) coordinates in the Fourier domain where $\smash{\vec{\xi} \cdot \hat{\vec{\psi}}(\xi) = 0}$ can be ensured by choosing a vectorial part without radial component.
To exploit this, we define our wavelets as $\smash{\hat{\vec{\psi}}(\xi)} = \hat{\psi}(\xi) \, \vec{\tau}$ where the vector component $\vec{\tau}$ is chosen such that it is tangential to $\smash{S_{\xi}^{d-1}}$ and $\hat{\psi}(\xi)$ is a scalar window function controlling the frequency localization.
We use bandlimited windows defined separably in polar or spherical coordinates as $\hat{\psi}(\xi) = \hat{\gamma}(\theta) \, \hat{h}(\vert \xi \vert)$ and which are hence compatible with the divergence freedom constraint.
Among other things, this enables us to obtain closed form expressions for the wavelets in the spatial domain.
%Spherical (or polar) coordinates provide hence a natural parametrization for our construction since $\smash{\vec{\xi} \cdot \hat{\vec{u}}(\xi) = 0}$ can be ensured by simply choosing a vector field without radial component.
%The frequency windows describing our wavelets are hence defined in polar coordinates, which corresponds to the polar wavelets recently introduced by Unser and co-workers~\cite{Chenouard2012,Unser2013,Ward2014}.
The construction is particular simple in $\mathbb{R}^2$ where the angular basis vector $\vec{e}_{\theta_{\xi}}$ spans all non-radial vector fields, that is all whose inverse Fourier transform is divergence free, and hence our wavelets are given by $\hat{\psi}(\xi) = -i \,\hat{\gamma}(\theta_{\xi}) \, \hat{h}(\vert \gamma \vert) \,  \vec{e}_{\theta_{\xi}}$.

Since we use bandlimited window functions, our wavelets do not have compact support in the spatial domain.
One hence typically needs a large number of frame functions around the actual region of interest and it also implies that the filter taps for the fast transform usually have to be truncated, resulting in limited accuracy.
Nonetheless, our numerical results demonstrate that one can work efficiently with our wavelets and using only algorithms that operate in the spatial domain where it is easier to exploit sparsity.

%\begin{figure}
%  \includegraphics[width=1.0\columnwidth]{figures/teaser.pdf}
%  \caption{\emph{Left:} A vector field $\vec{u}(x)$ is divergence free when its Fourier transform $\hat{\vec{u}}(\xi)$ is tangential to the frequency sphere $S_{\xi}^{d-1}$. We thus construct our wavelets so that it has no radial vector component and using window functions defined in spherical (or polar) coordinates. \emph{Right:} Isotropic and directional functions in the frequency (left) and spatial (right) domains.}
%  \label{fig:teaser}
%\end{figure}


% Scalar wavelets defined in polar coordinates have recently been introduced by Unser and co-workers~\cite{Chenouard2012,Unser2013,Ward2014} and these provide the basis for our construction.
Divergence free wavelets were first developed in the 1980s for four-dimensional spacetime~\cite{Federbush1986,Federbush1987a,Federbush1988}.
In the 1990s, several compactly supported, divergence-free wavelets for Euclidean space were proposed~\cite{LemarieRieusset1992,Battle1993,Battle1994,Urban1995}.
In comparison to our construction, the definitions of these wavelets are considerably more complicated and they do not provide well defined angular selectivity.
Our wavelets, in contrast, do not have compact support.
%Our wavelets furthermore benefit from a simple implementation using closed form expressions and fast transforms~\cite{Deriaz2005} although they are bandlimited in frequency space and hence non-compactly supported in space.
%In practice one therefore also typically truncates the filter taps for the fast transform, which incurs some error.
Closest to the present construction is recent work by Bostan, Unser and Ward~\cite{Bostan2015} who also proposed a tight, divergence free wavelet frame using window functions that are separable in polar (or spherical) coordinates.
In contrast to our approach, however, these authors enforce divergence freedom numerically by removing the radial frequency component of wavelets defined in Cartesian coordinates.
This makes an efficient spatial implementation of their wavelets difficult and prevents them from considering angular localization.
In the scalar setting, polar-separable windows and the resulting scalar polar wavelets have recently been studied systematically by Unser and co-workers~\cite{Chenouard2012,Unser2013,Ward2014}, extending previous work on steerable wavelets.
These results provide an important basis for our work.

%Interestingly, some of the first wavelets in the 1980s were divergence free~\cite{Federbush1986,Federbush1987a} although, to our knowledge, these have never been implemented.
%What did Urban exactly do? Can we relate to it more precisely? (But probably not too relevant for the venue).


==> macros.tex <==
% MISC

\allowdisplaybreaks

% theorems etc
% italic
\theoremstyle{plain}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
% non-italic
\newtheorem{algo}{Algorithm}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

% new empty set command which is prettier
\font\msbm = msbm10 at 12pt
\def\Emptyset{\hbox{\msbm \char 63}}

% General typesetting
%\newcommand{\bemph}[1]{{\textbf{\emph{#1}}}}
\newcommand{\bemph}[1]{{\textbf{{#1}}}}
\newcommand{\dbar}[1]{{\bar{\bar{#1}}}}
%\def\tighteq{\setlength{\belowdisplayskip}{5pt}\setlength{\abovedisplayskip}{5pt}}
\def\tighteq{\abovedisplayskip=6pt plus 3pt minus 3pt 
\abovedisplayshortskip=3pt plus 2pt minus 2pt
\belowdisplayskip=6pt plus 3pt minus 3pt 
\belowdisplayshortskip=3pt plus 2pt minus 2pt}
\def\es{\hspace{0.015in}}

% LIGHT TRANSPORT
\def\outd{_{\scriptscriptstyle{+}}}    % incoming direction
%\def\ind{_{\scriptscriptstyle{-}}}    % outgoing direction
\def\d{\mathrm{d}}
\def\dd{\mathrm{d}}
\def\Den{\mathrm{Den}}
\def\E{\mathbf{E}}
\def\V{\mathrm{V}}  
\def\W{\mathrm{W}}  
\def\U{\mathrm{U}}  
\def\T{T}  
\def\St{S^2}
\def\circle{S^1}
\def\Sp{\mathbb{S}\outd^2}
%\def\Sm{\mathbb{S}\ind^2}
\def\Ht{\mathbb{H}^2}
\def\Hp{\mathcal{H}\outd^2}
%\def\Hm{\mathcal{H}\ind^2}
\def\Z{\mathbb{Z}}
\def\R{\mathbb{R}}
\def\C{\mathbb{C}}
\def\M{\mathcal{M}}
\def\N{\mathcal{N}}
\def\K{\mathcal{K}}
\def\H{\mathcal{H}}    % general Hilbert space
\def\G{\mathcal{G}}    % second general Hilbert space
\def\Hk{\mathcal{H}_k}  % reproducing kernel Hilbert space
\def\F{\mathcal{F}}  %
\def\bs{\boldsymbol}
\def\sa{\bs\omega}
\def\bsa{\bar{\bs\omega}}     % basic cosine weighted solid angle measure
\def\sap{\bs\varpi}           % solid angle primed
\def\brho{\bar{\rho}}         % basic bidirectional distribution function
\def\T{\mb{T}}                % transport operator
\def\P{\mb{P}}                % shading operator
\def\r{\mn{r}}                % ray casting function
\def\p{\mb{p}}                % path
\def\g{\mn{g}}                % geometry function
\def\v{\mn{v}}                % visibility function
\def\n{\mb{n}}                % normal
\def\nn{\bar{\mb{n}}}         % normalized normal
\def\dx{\d\mb{x}}            % standard differential in Euclidean space
\def\dbx{\d\bar{\mb{x}}}     % barred standard differential in Euclidean space
\def\llangle{\langle \langle}     % left bracket for inner product of dual space
\def\rrangle{\rangle \rangle}     % left bracket for inner product of dual space
\def\dAo{\dA_{\scriptscriptstyle{\bot}}}    % outgoing direction
\def\w{\omega}
\def\hnu{\hat{\nu}}
\def\bw{\bar{\omega}}
\def\eps{\epsilon}
% composition of functions (a slightly smaller circ)
\def\comp{\, {\scriptscriptstyle{^\circ}} \,}
% Don't use DeclareMathOperator
\def\sinc{\textrm{sinc}}
\def\ip{\mathrm{i}}

% pre-radiance
\def\tell{\tilde{\ell}}
% coordinate function of phase space light energy density
\def\L{\ell}

%bold greek letters
\def\balpha{\boldsymbol \alpha}
\def\blambda{\boldsymbol \lambda}
\def\bgamma{\boldsymbol \gamma}
\def\bpsi{\boldsymbol \psi}
\def\bbeta{\boldsymbol \beta}
\def\bell{\boldsymbol \ell}

% brackets
% double angle brackets 
\def\llangle{\langle \! \langle}
\def\rrangle{\rangle \! \rangle}

%\DeclareMathOperator*{\vdiv}{div}
\def\vdiv{\mathrm{div}}
\DeclareMathOperator*{\vgrad}{grad}
\DeclareMathOperator*{\vcurl}{curl}
\DeclareMathOperator*{\sign}{sgn}
\DeclareMathOperator*{\supp}{supp}
\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator*{\spann}{span}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\tr}{tr}
\DeclareMathOperator*{\codim}{codim}
\DeclareMathOperator*{\cond}{cond \!}
\DeclareMathOperator*{\card}{card}
\DeclareMathOperator*{\BV}{BV}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\interior}{int}
\DeclareMathOperator*{\kernel}{ker}
\DeclareMathOperator*{\range}{ran}
\DeclareMathOperator*{\ind}{ind}
\def\fromto{\leftrightarrow}
\def\colvec#1#2#3{\left( \begin{array}{c} #1 \\ #2 \\ #3 \end{array} \right)}
\def\mb#1{\mathbf{#1}}
\def\mn#1{\mathrm{#1}}
\def\mf#1{\mathfrak{#1}}
\def\mc#1{\mathcal{#1}}
\def\bs{\boldsymbol}
\def\sa{\bs\omega}       % solid angle
\def\rsm{\bs\lambda}     % ray space measure
\def\drsm{\d \bar{\bs\lambda}}    % ray space measure
\def\rect{\mathrm{rect}}
\def\transversal{\pitchfork}

\def\poyntn{\bar{\mathbf{s}}}      % normalized direction of Poynting 2-form

% Canonical diffeomorphism group
\def\Dgc{\mathrm{Diff}_{\mathrm{can}}}
% Canonical diffeomorphisms generated by Hamiltonian vector fields
\def\Dgham{\mathrm{Diff}_{\mathrm{Ham}}}
% Canonical diffeomorphism group on slit cotangent bundle T*Q \ {0} preserving the contact structure
\def\Dgs{\mathrm{Diff}_{\mathrm{can}}^{\theta} \left(T^*Q \! \setminus \! \{ 0 \} \right)}
% (General) diffeomorphism group
\def\Dg{\mathrm{Diff}}
% Volume preserving diffeomorphism group
\def\Dgv{\mathrm{Diff}_{\mu}}
% Contact form preserving diffeomorphism group
\def\Dgcon{\mathrm{Diff}_{\mathrm{con}}}
% Rotation groups
\newcommand{\SO}[1]{\ensuremath{\mathrm{SO}(#1)}}
% Lie algebras of rotation groups
\newcommand{\so}[1]{\ensuremath{\mathfrak{so}(#1)}}
% Dual Lie algebras of rotation groups
\newcommand{\dso}[1]{\ensuremath{\mathfrak{so}^*(#1)}}
% general linear group
\newcommand{\GL}[1]{\ensuremath{\mathrm{GL}(#1,\R)}}
% Momentum map
\def\mmap{\ensuremath \mathbf{J}}
% General Lie algebra
\def\la{\ensuremath \mathfrak{g}}
% Lie derviative
\def\Lie{\pounds}
% Adjoint action
\def\Ad{\mathrm{Ad}}
% Infinitesimal adjoint action
\def\ad{\mathrm{ad}}
% configuration space
%\def\Q{\mathcal{Q}}
\def\Q{Q}
% phase space
%\def\P{\mathcal{P}}
\def\P{P}
% local representative
\def\lr{\mathrm{lr}}
% Lie algebra
\def\g{\mathfrak{g}}
% Lie algebra of Diff_can
\def\gcan{\mathfrak{s}}
% Lie group
\def\G{G}
% space of Hamiltonian vector fields
\def\XHam{\mathfrak{X}_{\mathrm{Ham}}}

\newcommand{\dtp}[1]{\ensuremath{\frac{\partial #1}{\partial t}}}
\newcommand{\dpp}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\newcommand{\dnabla}[1]{\ensuremath{\nabla_{\hspace{-0.02in} #1}}}
\newcommand{\coadjoint}[2]{\ensuremath{\textrm{ad}_{#1}^{*} #2}}
% small minus sign for exponents (e.g. inverse operators)
%\def\ms{\textrm{--}}
\def\ms{-}

% no slip boundary conditions for kinetic theory
\def\bcondk{\parallel\!)}

% red / blue / green text 
% (use providecommand to avoid problems with the red / blue / green commands
% defined in the pstricks package)
\providecommand{\red}[1]{ {\color{red} #1}}
\providecommand{\blue}[1]{ {\color{blue} #1}}
\providecommand{\green}[1]{ {\color{green} #1}}
\providecommand{\white}[1]{ {\color{white} #1}}
% Numbers
\def\century{^\textrm{th}}
\def\expth{^\textrm{th}}

% short arrow
\def\sa{\hspace{-0.025in}\shortrightarrow\hspace{-0.025in}}
\def\sar{\hspace{-0.025in}\shortleftarrow \hspace{-0.1in}\shortrightarrow\hspace{-0.025in}}

\usepackage{mathtools}     %in order to write Meijer G-functions
\usepackage{suffix}         %in order to write Meijer G-functions
\usepackage{relsize}

%Meijer G-functions
\DeclarePairedDelimiterX\MeijerM[3]{\lparen}{\rparen}%                    
{\begin{smallmatrix}#1 \\ #2\end{smallmatrix}\delimsize\vert\,#3}     

\newcommand\MeijerG[8][]{%                           
  G^{\,#2,#3}_{#4,#5}\MeijerM[#1]{#6}{#7}{#8}}       

\WithSuffix\newcommand\MeijerG*[7]{%                 
  G^{\,#1,#2}_{#3,#4}\MeijerM*{#5}{#6}{#7}}          




